The subtlety of Ly-a photons: changing the expected range of the 21-cm signal

We present the evolution of the 21-cm signal from cosmic dawn and the epoch of reionization (EoR) in an upgraded model including three subtle effects of Ly-a radiation: Ly-a heating, CMB heating (mediated by Ly-a photons), and multiple scattering of Ly-a photons. Taking these effects into account we explore a wide range of astrophysical models and quantify the impact of these processes on the global 21-cm signal and its power spectrum at observable scales and redshifts. We find that, in agreement with the literature, Ly-a and CMB heating raise the gas temperature by up to $\mathcal{O}(100)$ degrees in models with weak X-ray heating and, thus, suppress the predicted 21-cm signals. Varying the astrophysical parameters over broad ranges, we find that in the upgraded model the absorption trough of the global signal reaches a lowest floor of $-165$ mK at redshifts $z\approx 15-19$. This is in contrast with the predictions for a pure adiabatically cooling Universe, for which the deepest possible absorption is a monotonically decreasing function of cosmic time and is $-178$ mK at $z = 19$ and $-216$ mK at $z=15$, dropping to even lower values at lower redshifts (e.g. $-264$ mK at $z = 10$). With the Ly-a and CMB heating included we also observe a strong suppression in the low-redshift power spectra, with the maximum possible power (evaluated over the ensemble of models) attenuated by a factor of $6.6$ at $z=9$ and $k = 0.1$ Mpc$^{-1}$. Finally, we find that at high redshifts corresponding to cosmic dawn, the heating terms have a subdominant effect while multiple scattering of Ly-a photons is important, leading to an amplification of the power spectrum by a factor of $\sim 2-5$.

==> parameters.tex <==

\begin{table}
\begin{center}


\tiny
\begin{tabular}{l|ccc}

\toprule
Parameter & Allowed range  & Description     \\
\midrule
$f_*$ & 0.0001 - 0.5  &  Star formation efficiency \\
$V_c$ & 4.2 - 100 km s$^{-1}$  & Circular velocity (minimum mass for star formation, Eqn. \ref{eqn:vc})\\
$f_X$ &  $10^{-4}$ - $10^{3}$  & X-ray production efficiency\\
$\alpha$ &  1 - 1.5  & X-ray SED slope\\
$\nu_{\rm min}$ &  0.1 - 3 keV  & X-ray SED minimum frequency\\
$\tau$ &  0.033 - 0.089  & Optical depth to reionization\\
R$_{\rm MFP}$ &  10 - 70 Mpc  & Mean free path for ionizing photons\\



 \bottomrule
\end{tabular}
\caption{The parameters of our simulation and their allowed ranges. The X-ray SED parameters $\alpha$ and $\nu_{\rm min}$ represent a power law with a cutoff. We also consider the realistic X-ray binary (XRB) SED from \citet{fragos13}, in which case  $\alpha$ and $\nu_{\rm min}$ are not used. }
\label{tab:parameters}

\large
\end{center}
\end{table}
